Bayesian inference of an uncertain generalized diffusion operator

This paper defines a novel Bayesian inverse problem to infer an infinite-dimensional uncertain operator appearing in a differential equation, whose action on an observable state variable affects its dynamics. Inference is made tractable by parametrizing the operator using its eigendecomposition. The plausibility of operator inference in the sparse data regime is explored in terms of an uncertain, generalized diffusion operator appearing in an evolution equation for a contaminant's transport through a heterogeneous porous medium. Sparse data are augmented with prior information through the imposition of deterministic constraints on the eigendecomposition and the use of qualitative information about the system in the definition of the prior distribution. Limited observations of the state variable's evolution are used as data for inference, and the dependence on the solution of the inverse problem is studied as a function of the frequency of observations, as well as on whether or not the data is collected as a spatial or time series.

==> Makefile <==
#vectorsources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.dia' -o -name '*.eps' -o -name '*.m' -o -name '*.pdf' -o -name '*.ps' -o -name '*.py' -o -name '*.svg' 2>/dev/null)
#rastersources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.jpg' -o -name '*.gif' 2>/dev/null)
readysources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.png' -o -name '*.pdf' -o -name '*mpg' -o -name '*.mpeg' 2>/dev/null)
#texsource := $(wildcard abstract.tex paper.tex poster.tex proposal.tex report.tex talk.tex)
texsource := $(wildcard paper.tex poster.tex proposal.tex report.tex talk.tex)

#vectorfigs := $(shell echo ' ' $(patsubst %_fm.eps,%.eps,$(vectorsources)) ' ' | sed -e 's> \(../common/\)*raw> >g' -e 's/\.[^. ]* /.pdf /g')
#rasterfigs := $(shell echo ' ' $(rastersources) ' ' | sed -e 's> \(../common/\)*raw> >g' -e 's/\.[^. ]* /.png /g')
readyfigs := $(shell echo ' ' $(readysources) ' ' | sed -e 's> \(../common/\)*raw> >g')
figsources := $(vectorsources) $(rastersources) $(readysources)
figures := $(vectorfigs) $(rasterfigs) $(readyfigs)
dirname  := $(shell basename $(shell pwd))
ifeq ($(words $(texsource)),'1')
    texfinal := $(dirname).pdf
    texroot   = $(patsubst %.pdf,%,$(1))
else
    texfinal := $(patsubst %.tex,$(dirname)-%.pdf,$(texsource))
    texroot   = $(patsubst $(dirname)-%,%,$(patsubst %.pdf,%,$(1)))
endif

bibfiles := $(wildcard *.bib)
styfiles := $(wildcard *.sty ../common/*.sty)
clsfiles := $(wildcard *.cls ../common/*.cls)

alldeps := *.tex $(bibfiles) $(figures) $(figsources) $(clsfiles) $(styfiles)

BIBTEX     ?= bibtex
PDFLATEX   ?= pdflatex
LATEX      ?= latex
PYTHON     ?= python
OCTAVE     ?= octave
INKSCAPE   ?= inkscape
FRAGMASTER ?= fragmaster

MYPDFLATEX   = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(PDFLATEX) -halt-on-error -interaction=nonstopmode
MYLATEX      = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(LATEX) -halt-on-error -interaction=nonstopmode
MYFRAGMASTER = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(FRAGMASTER)

.PHONY: all figures clean cleanlatex cleanfigs

all: $(texfinal)

figures: $(figures)

continuous: all
	while true; do \
	  inotifywait -e close_write -e delete_self -e move $(alldeps) || break; \
          $(MAKE) all; \
        done

$(texfinal): $(alldeps)
	if ls *.bib 2>&1; then $(MYPDFLATEX) -draftmode $(call texroot,$@); fi
	if (ls *.bib 2>&1 && ls $(call texroot,$@).aux 2>&1); then $(BIBTEX) $(call texroot,$@); fi
	$(MYPDFLATEX) -draftmode $(call texroot,$@) && $(MYPDFLATEX) -draftmode $(call texroot,$@) && $(MYPDFLATEX) $(call texroot,$@)
	if [ "$@" != "$(call texroot,$@).pdf" ]; then mv "$(call texroot,$@).pdf" "$@"; fi

clean: cleanlatex cleanfigs

cleanlatex:
	rm -f $(patsubst %.tex, %.aux, $(wildcard *.tex))
	#rm -f $(foreach ext,.bbl .blg .log .dvi .nav .nlo .out .pdf .snm .spl .toc .vrb Notes.bib,$(patsubst %.tex,%$(ext),$(texsource)))
	rm -f $(foreach ext, .bbl .blg .log .dvi .nav .nlo .out .thm .pdf .snm .spl .toc .vrb .cb .cb2 Notes.bib,$(patsubst %.tex,%$(ext),$(texsource)))
	rm -f $(texfinal)

cleanfigs:
	rm -rf figs/

figs/%.pdf: rawfigs/%.dia
	@mkdir -p $(dir $@)
	dia -t eps-builtin -e $?_roytemp.eps $? && epstopdf $?_roytemp.eps -o=$@
	@rm -f $?_roytemp.eps

figs/%.pdf: rawfigs/%.eps
	@mkdir -p $(dir $@)
	epstopdf $? -o=$@ || (rm $@; exit 1)

figs/%.pdf: rawfigs/%_fm rawfigs/%_fm.eps  # fragmaster(1) with optional control file
	@mkdir -p $(dir $@)
	@(test -f rawfigs/fragmaster.dfm && (cd $(dir $@) && ln -sf -t . ../rawfigs/fragmaster.dfm) || true)
	@(cd $(dir $@) && ln -sf -t . $(addprefix ../,$+) && $(MYFRAGMASTER))

figs/%.pdf: rawfigs/%.m
	@mkdir -p $(dir $@)
	@cd $(dir $?) && $(OCTAVE) $(notdir $?)
	@(test -f $(dir $?)/$*.eps && (epstopdf $(dir $?)/$*.eps -o=$@; rm -f $(dir $?)/$*.eps) || true)
	@(test -f $(dir $?)/$*.pdf && mv $(dir $?)/$*.pdf $@ || true)

figs/%.pdf: rawfigs/%.py
	@mkdir -p $(dir $@)
	@cd $(dir $?) && $(PYTHON) $(notdir $?)
	@(test -f $(dir $?)/$*.eps && (epstopdf $(dir $?)/$*.eps -o=$@; rm -f $(dir $?)/$*.eps) || true)
	@(test -f $(dir $?)/$*.pdf && mv $(dir $?)/$*.pdf $@ || true)

figs/%.pdf: rawfigs/%.ps
	@mkdir -p $(dir $@)
	ps2pdf $? $@

#figs/%.pdf: rawfigs/%.png
#       convert $? $@

figs/%.pdf: rawfigs/%.svg
	@mkdir -p $(dir $@)
	$(INKSCAPE) $? -z --export-pdf=$@

figs/%.png: rawfigs/%.jpg
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: ../common/rawfigs/%.jpg
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: rawfigs/%.gif
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: ../common/rawfigs/%.gif
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.mpeg: rawfigs/%.mpeg
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.mpg: rawfigs/%.mpg
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: rawfigs/%.pdf
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.png: rawfigs/%.png
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: ../common/rawfigs/%.pdf
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.png: ../common/rawfigs/%.png
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: ../common/rawfigs/%.eps
	@mkdir -p $(dir $@)
	epstopdf $? -o=$@

figs/%.pdf: ../common/rawfigs/%.ps
	@mkdir -p $(dir $@)
	ps2pdf $? $@

figs/%.pdf: ../common/rawfigs/%.svg
	@mkdir -p $(dir $@)
	$(INKSCAPE) $? -z --export-pdf=$@

